Analysis of the Evolution of a Multi-Ribbon Flare and Failed Filament Eruption

How filaments form and erupt are topics about which solar researchers have wondered since more than a century and that are still open to debate. We present observations of a filament formation, its failed eruption, and the associated flare (SOL2019-05-09T05:51) that occurred in active region (AR) 12740 using data from SDO, STEREO-A, IRIS, and NSO/GONG. AR 12740 was a decaying region formed by a very disperse following polarity and a strong leading spot, surrounded by a highly dynamic zone where moving magnetic features (MMFs) were seen constantly diverging from the spot. Our analysis indicates that the filament was formed by the convergence of fibrils at a location where magnetic flux cancellation was observed. Furthermore, we conclude that its destabilization was also related to flux cancellation associated to the constant shuffling of the MMFs. A two-ribbon flare occurred associated to the filament eruption; however, because the large-scale magnetic configuration of the AR was quadrupolar, two additional flare ribbons developed far from the two main ones. We model the magnetic configuration of the AR using a force-free field approach at the AR scale size. This local model is complemented by a global potential-field source-surface one. Based on the local model, we propose a scenario in which the filament failed eruption and flare are due to two reconnection processes, one occurring below the erupting filament, leading to the two-ribbon flare, and another one above it between the filament flux-rope configuration and the large-scale closed loops. Our computation of the reconnected magnetic flux added to the erupting flux rope, compared to that of the large-scale field overlying it, lets us conclude that the latter was large enough to prevent the filament eruption. A similar conjecture can be drawn from the computation of the magnetic tension derived from the global field model.

==> MS_labels.tex <==


\sect{intro}
\sect{data}
\sect{events}
   \sect{obs_B}
   \sect{filform}
   \sect{flare}
   \sect{filerup}
     \sect{}
     \sect{}
\sect{model}
   \sect{overview}
   \sect{local_model}
   \sect{scenario}
   \sect{global_model}
\sect{discussion}

 1 Fig.~\ref{fulldisk}
 2 Fig.~\ref{twoCRs}
 3 Fig.~\ref{MMF}
 4 Fig.~\ref{cancelflux}
 5 Fig.~\ref{formation}
 6 Fig.~\ref{AIA}
 7 Fig.~\ref{IRIS}
 8 Fig.~\ref{stereo}
 9 Fig.~\ref{Halphaevolution}
10 Fig.~\ref{evolution171}
11 Fig.~\ref{timeslice}
12 Fig.~\ref{preflare}
13 Fig.~\ref{flare}
14 Fig.~\ref{posflare}
15 Fig.~\ref{sketch}
16 Fig.~\ref{AIA-PFSS}
17 Fig.~\ref{tension}

 %%% labels
 Fil$_1$  Fil$_2$
 L$_1$  L$_2$  L$_3$
 
Evolution:
 tStartFlare    5:40 UT  
   
% Commands for figures, sections & equations,
\newcommand{\fig}[1]{Figure~\ref{fig_#1}}
\newcommand{\figS}[1]{Figures~\ref{fig_#1}}
\newcommand{\figs}[2]{Figures~\ref{fig_#1} and \ref{fig_#2}}
\newcommand{\figss}[2]{Figures~\ref{fig_#1}-\ref{fig_#2}}
\newcommand{\sect}[1]{Section~\ref{sect_#1}}
\newcommand{\sects}[2]{Sections~\ref{sect_#1} and~\ref{sect_#2}}
\newcommand{\eq}[1]{Equation~(\ref{eq_#1})}
\newcommand{\eqs}[2]{Equations~(\ref{eq_#1}) and (\ref{eq_#2})}
\newcommand{\eqss}[2]{Equations~(\ref{eq_#1}) - (\ref{eq_#2})}
\newcommand{\eqsss}[3]{Equations~(\ref{eq_#1}), (\ref{eq_#2}) and (\ref{eq_#3})}
\newcommand{\tab}[1]{Table~\ref{tab_#1}}
\newcommand{\BE}{\begin{equation}}
\newcommand{\EE}{\end{equation}}
\newcommand{\BA}{\begin{eqnarray}}
\newcommand{\EA}{\end{eqnarray}}

% General definitions for derivatives
\newcommand{\f}[2]{{\ensuremath{\mathchoice%
        {\dfrac{#1}{#2}}
        {\dfrac{#1}{#2}}
        {\frac{#1}{#2}}
        {\frac{#1}{#2}}
        }}}
\newcommand{\Int}[2]{\ensuremath{\mathchoice%
        {\displaystyle\int_{#1}^{#2}}
        {\displaystyle\int_{#1}^{#2}}
        {\int_{#1}^{#2}}
        {\int_{#1}^{#2}}
        }}
\newcommand{\curl}{ {\bf \nabla } \times}
\newcommand{\rmd}{{\rm d }}
\renewcommand{\div}[1]{ {\bf \nabla}. #1 }
\newcommand{\grad}{  {\bf \nabla} }
%\newcommand{\pardiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pder}[2]{\f{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\f{\rmd \, #1}{\rmd \, #2}}

% General definitions of symbols 
\newcommand{\arcsec}{''} 
\newcommand{\degree}{^\circ} 
\newcommand{\kms}{km s$^{-1}$} %{km/s} 
\newcommand{\Rsun}{$R_{\odot}$}  
\newcommand{\uvec}[1]{\hat{\bf #1}}
%\renewcommand{\vec}[1]{ \textit{\textbf{#1}} }

% text
\newcommand{\cf}{\textit{cf.}}
\newcommand{\eg}{\textit{e.g.,}}
\newcommand{\etal}{\textit{et al.}}
\newcommand{\ie}{\textit{i.e.,}}
\newcommand{\insitu}{\textit{in situ}}
\newcommand{\vs}{\textit{vs}}
\newcommand{\vv}{\textit{v.v.}}
\newcommand{\de}{$\Delta$} 
\newcommand{\ha}{H$\alpha$}



==> sola_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{et al.}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})


